Are Abstracts Enough for Hypothesis Generation?

The potential for automatic hypothesis generation (HG) systems to improve research productivity keeps pace with the growing set of publicly available scientific information. But as data becomes easier to acquire, we must understand the effect different textual data sources have on our resulting hypotheses. Are abstracts enough for HG, or does it need full-text papers? How many papers does an HG system need to make valuable predictions? How sensitive is a general-purpose HG system to hyperparameter values or input quality? What effect does corpus size and document length have on HG results? To answer these questions we train multiple versions of knowledge network-based HG system, Moliere, on varying corpora in order to compare challenges and trade offs in terms of result quality and computational requirements. Moliere generalizes main principles of similar knowledge network-based HG systems and reinforces them with topic modeling components. The corpora include the abstract and full-text versions of PubMed Central, as well as iterative halves of MEDLINE, which allows us to compare the effect document length and count has on the results. We find that, quantitatively, corpora with a higher median document length result in marginally higher quality results, yet require substantially longer to process. However, qualitatively, full-length papers introduce a significant number of intruder terms to the resulting topics, which decreases human interpretability. Additionally, we find that the effect of document length is greater than that of document count, even if both sets contain only paper abstracts. Reproducibility: Our code and data are available at github.com/jsybran/moliere, and bit.ly/2GxghpM respectively.

==> sections/futurework.tex <==
\section{Future Work}\label{sec:futurework}

\subsection{Mapping Data to Prediction Potential}

As the size of the labeled data for hypothesis generation increases, it would be good to build models that estimate data sources and the phrase quality for its potential to make predictions.
To gain insight now, we trained and ran on extremes (abstracts only, abstracts with full-text model training data, and full texts), but it would be beneficial to determine which sections are most relevant.

Another question to ask is how many abstracts would be needed to match full-texts in their ability to create LBD models. It may be the case that the unique phrases would be mostly captured by abstracts at some point. 



